GERestaurant: A German Dataset of Annotated Restaurant Reviews for Aspect-Based Sentiment Analysis

We present GERestaurant, a novel dataset consisting of 3,078 German language restaurant reviews manually annotated for Aspect-Based Sentiment Analysis (ABSA). All reviews were collected from Tripadvisor, covering a diverse selection of restaurants, including regional and international cuisine with various culinary styles. The annotations encompass both implicit and explicit aspects, including all aspect terms, their corresponding aspect categories, and the sentiments expressed towards them. Furthermore, we provide baseline scores for the four ABSA tasks Aspect Category Detection, Aspect Category Sentiment Analysis, End-to-End ABSA and Target Aspect Sentiment Detection as a reference point for future advances. The dataset fills a gap in German language resources and facilitates exploration of ABSA in the restaurant domain.

==> old/03_acquisition.tex <==
\section{Data Acquisition}

To gather German-language restaurant reviews, Tripadvisor was selected as the data source. The five restaurants with the most customer reviews in the 25 most densely populated German cities as of 2022\footnote{German Federal Statistical Office, population and population density as of December 31, 2022: \url{https://www.destatis.de/DE/Themen/Laender-Regionen/Regionales/Gemeindeverzeichnis/Administrativ/05-staedte.html}} were considered, covering a wide spectrum of restaurant types, including regional, Italian, Asian, and fast-food venues. In the course of the COVID-19 pandemic, restaurant reviews were influenced by the associated hygiene measures. Hence, all reviews posted during a period without mandated COVID-19 hygiene restrictions, specifically from October 15, 2022, to October 15, 2023, were taken into account.

Overall, a total of 3,212 user reviews with a German language label on Tripadvisor were collected. The reviews were segmented into 13,426 sentences using the NLTK Tokenizer \cite{loper2002nltk}. It was observed that, despite the German language code label, some sentences were in languages other than German. Due to this, \textit{langdetect}\footnote{\url{https://pypi.org/project/langdetect}} was employed to ascertain the language of each sentence, leading to the rejection of 631 sentences which resulted in a total of 12,795 sentences in German. 

Ultimately, the sentences underwent an anonymization process. Named entity recognition (NER) was employed using \textit{spaCy}\footnote{\url{https://pypi.org/project/spacy}} (\textit{de\_core\_news\_lg} model) to replace locations, personal names, and time-related references with anonymized placeholders \textit{"LOC"}, \textit{"PERSON"} and \textit{"DATE"}. Subsequently, regular expressions were employed to substitute any mentions of the restaurant's name in the sentences with the placeholder \textit{"RESTAURANT\_NAME"}.

